Training and Evaluating Causal Forecasting Models for Time-Series

Deep learning time-series models are often used to make forecasts that inform downstream decisions. Since these decisions can differ from those in the training set, there is an implicit requirement that time-series models will generalize outside of their training distribution. Despite this core requirement, time-series models are typically trained and evaluated on in-distribution predictive tasks. We extend the orthogonal statistical learning framework to train causal time-series models that generalize better when forecasting the effect of actions outside of their training distribution. To evaluate these models, we leverage Regression Discontinuity Designs popular in economics to construct a test set of causal treatment effects.

==> sections/background.tex <==



As mentioned earlier, the forecasts provide information for decision making. Hence, it is mandatory for such forecasts to rely on causal links. If not, the operator will not use the forecast as it can not be trusted for rarely seen in dataset. Traditionally, deep learning models suppose that the training data are randomly sampled from an hidden distribution. Nonetheless, in some use cases such as econometric or health, the training data are not randomly sampled. Indeed, the treatment assignment depends on other counterfactuals. Those dynamics are hard to learn from scratch for a deep learning. Without any consideration for this matter, a model might learn the wrong correlation between the treatment and the outcome. 

\begin{figure}[h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.44]{images/background/Daily_wrong.png}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[scale=0.3]{images/background/histograme_10_wrong.png}
\end{subfigure}
\caption{(a):Forecasting the daily demand on train tickets. The blue line is the ground truth, the orange one is the forecast for the prices applied in real life, the green curve is the forecast for an increase of 30\% of prices (b): CATE distribution between the real price and the next possible price  \tc{I had to change the meaning of the increase bcz vector models do not see all prices between 10 and 100€, thus increasing prices by 10\% returns crazy values for vector causal models}\ml{Yes! I plan to port this under the heading "The need for causal forecasting": the goal of this background is to introduce notation, formalize the prob, and show why we need causal things. Then we describe our approach. This section 2 should be quite formal, with precise definitions, assumptions, and results, more than long text. The text for high level intuition is mostly in the intro to S2 and each subsection, and then we just put lower-level intuition for the formalism/results in the rest} for three different models: a baseline TFT model, a standard Light Gradient Boosting Machine (LGBM) and a LGBM constrained to learn the monotonicity of the outcome with regard to the treatment}
\label{motivation}
\end{figure}



We see on figure \ref{motivation} an example where a model learns the wrong link between the treatment and the outcome. Increasing the value of prices leads to a bigger sales prediction which is the wrong behaviour. Indeed, the economic theory implies that the demand decreases when the prices increase. Nonetheless, the model has learned otherwise and infers that increasing the prices leads to bigger sales. On a more macro level, the histogram of the difference of prediction between the standard prices and the increased ones shows that the models haven't generalized for out of distribution treatments.
